New Developments in Cosmology

In this Thesis I discuss several recent results obtained using the CMB spectra measured by Planck and several other cosmological probes. Extensions of the $\Lambda$CDM model are studied, including the presence of an additional sterile neutrino (motivated by the short-baseline oscillation anomalies) and of a thermal axion. The degeneracies of the cosmological effects of these particles with the power spectrum of primordial perturbations are tested. We also show that the power spectrum of initial scalar perturbations can be degenerate with the presence of primordial non-Gaussianities, thus affecting the constraints on the non-Gaussianity parameter $f_{NL}$. Finally, an effective interaction between dark energy and dark matter is studied.

==> includes/scien_comm.tex <==
%!TeX root=main.tex
\newcommand{\prd}{Phys. Rev. D}
\newcommand{\jcap}{JCAP}
\newcommand{\apj}{ApJ}
\newcommand{\apjl}{ApJ, Letters}%{The Astrophysical Journal, Letters}
\newcommand{\apjs}{ApJ, Supplement}%{The Astrophysical Journal, Supplement}
\newcommand{\physrep}{Phys. Rep.}
\newcommand{\pasa}{PASA}%{Publications of the Astronomical Society of Australia}
\newcommand{\mnras}{MNRAS}
\newcommand{\nar}{NAR}%{New Astronomy Reviews}
\newcommand{\pasp}{PASP}%{Publications of the Astronomical Society of the Pacific}
\newcommand{\araa}{ARA\&A}%{Annual Review of Astronomy \& Astrophysics}
\newcommand{\zap}{Zeitschrift f{\"u}r Astrophysik}
\newcommand{\aap}{A\&A}
